Nano-Hall sensors with granular Co-C

We analyzed the performance of Hall sensors with different Co-C ratios, deposited directly in nano-structured form, using $Co_2(CO)_8$ gas molecules, by focused electron or ion beam induced deposition. Due to the enhanced inter-grain scattering in these granular wires, the Extraordinary Hall Effect can be increased by two orders of magnitude with respect to pure Co, up to a current sensitivity of $1 \Omega/T$. We show that the best magnetic field resolution at room temperature is obtained for Co ratios between 60% and 70% and is better than $1 \mu T/Hz^{1/2}$. For an active area of the sensor of $200 \times 200 nm^2$, the room temperature magnetic flux resolution is $\phi_{min} = 2\times10^{-5}\phi_0$, in the thermal noise frequency range, i.e. above 100 kHz.

==> a <==
\relax 
\citation{Sandhu}
\citation{Freitas-MRsensors}
\citation{Dolabdjian,Novoselov,Matveev-nanoHall}
\citation{Ivo-ReviewFebid}
\citation{Lau}
\citation{deTeresa-highpurity}
\citation{Giovanni-FebidHall}
\citation{Berger,Fert}
\citation{Ivo-TEM,Ivo-Conanocrystals}
\citation{Park}
\citation{Denardin}
\citation{Brouers}
\citation{Socolovsky}
\citation{PAKHOMOV}
\newlabel{FirstPage}{{}{1}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {I}Introduction}{1}{}}
\newlabel{eq1}{{1}{1}{}{}{}}
\citation{Laurent}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Hall sensors with different designs fabricated by FEBID with CO$_2$(CO)$_8$: (a) thin active area, (b) uniform thickness}}{2}{}}
\newlabel{Fig1}{{1}{2}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {II}Experimental}{2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces  Hall voltage as a function of the applied magnetic field for: (a) typical FEBID sensor, fitted with the Langevin Equation (2{}{}{}\hbox {}), (b) typical FIBID sensor, with linear fits at saturation (OH) and about zero field (EHE) as in Equation (1{}{}{}\hbox {})}}{2}{}}
\newlabel{Fig2}{{2}{2}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {III}Hall characterization}{2}{}}
\citation{Giovanni-HallDevices}
\@writefile{toc}{\contentsline {subsection}{\numberline {A}Langevin superparamagnetism}{3}{}}
\newlabel{Langevin}{{2}{3}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {B}Extraordinary Hall Effect}{3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {C}Saturation Field}{3}{}}
\newlabel{Bsat}{{3}{3}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Saturation field $B_\mathrm  {sat}$ as a function of: (a) Co atomic concentration, (b) the inverse of the parameter a, from Equation 2{}{}{}\hbox {}, proportional to the radius $r$ as in Equation 3{}{}{}\hbox {} }}{3}{}}
\newlabel{Fig3}{{3}{3}{}{}{}}
\@writefile{toc}{\contentsline {section}{\numberline {IV}Sensor characterization}{3}{}}
\newlabel{Bmin}{{4}{3}{}{}{}}
\citation{munter}
\citation{Giovanni-HallDevices}
\citation{Dolabdjian}
\citation{Novoselov}
\bibdata{biblio}
\bibcite{Sandhu}{{1}{2006}{{Togawa et~al.}}{{Togawa, Sanbonsugi, Sandhu, Abe, Narimatsu, Nishio, and Handa}}}
\bibcite{Freitas-MRsensors}{{2}{2007}{{Freitas et~al.}}{{Freitas, Ferreira, Cardoso, and Cardoso}}}
\bibcite{Dolabdjian}{{3}{2002}{{Dolabdjian et~al.}}{{Dolabdjian, Qasimi, Bloyet, and Mosser}}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Magnetic field resolution and field sensitivity as a function of: (a) the Co atomic concentration, (b) the inverse of the parameter a }}{4}{}}
\newlabel{Fig4}{{4}{4}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {}Low field detection}{4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {}}{4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {V}Conclusions}{4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {}Acknowledgments}{4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {}References}{4}{}}
\bibcite{Novoselov}{{4}{2003}{{Novoselov et~al.}}{{Novoselov, Morozov, Dubonos, Missous, Volkov, Christian, and Geim}}}
\bibcite{Matveev-nanoHall}{{5}{2008}{{Matveev et~al.}}{{Matveev, Levashov, Volkov, Kononenko, Chernyh, Knjazev, and Tulin}}}
\bibcite{Ivo-ReviewFebid}{{6}{2008}{{Utke et~al.}}{{Utke, Hoffmann, and Melngailis}}}
\bibcite{Lau}{{7}{2002}{{Lau et~al.}}{{Lau, Chee, Thong, and Ng}}}
\bibcite{deTeresa-highpurity}{{8}{2009}{{Fernandez-Pacheco et~al.}}{{Fernandez-Pacheco, Teresa, Cordoba, and Ibarra}}}
\bibcite{Giovanni-FebidHall}{{9}{2005}{{Boero et~al.}}{{Boero, Utke, Bret, Quack, Todorova, Mouaziz, Kejik, Brugger, Popovic, and Hoffmann}}}
\bibcite{Berger}{{10}{1979}{{{L. Berger and G. Bergmann}}}{{}}}
\bibcite{Fert}{{11}{1992}{{Fert and Lottis}}{{}}}
\bibcite{Ivo-TEM}{{12}{2005}{{Utke et~al.}}{{Utke, Michler, Gasser, Santschi, Laub, Cantoni, Buffat, Jiao, and Hoffmann}}}
\bibcite{Ivo-Conanocrystals}{{13}{2004}{{Utke et~al.}}{{Utke, Bret, Laub, Buffat, Scandella, and Hoffmann}}}
\bibcite{Park}{{14}{2003}{{Park et~al.}}{{Park, Yoon, Kim, Kim, Yoon, Song, Volkov, Avilov, and Park}}}
\bibcite{Denardin}{{15}{2008}{{Knobel et~al.}}{{Knobel, Nunes, Socolovsky, De~Biasi, Vargas, and Denardin}}}
\bibcite{Brouers}{{16}{1997}{{Brouers et~al.}}{{Brouers, Granovsky, Sarychev, and Kalitsov}}}
\bibcite{Socolovsky}{{17}{2005}{{Socolovsky et~al.}}{{Socolovsky, Oliveira, Denardin, Knobel, and Torriani}}}
\bibcite{PAKHOMOV}{{18}{1995}{{PAKHOMOV et~al.}}{{PAKHOMOV, YAN, and ZHAO}}}
\bibcite{Laurent}{{19}{2009}{{{L Bernau and M S Gabureac and I Utke and and J Michler P Hoffman}}}{{}}}
\bibcite{Giovanni-HallDevices}{{20}{2003}{{Boero et~al.}}{{Boero, Demierre, Besse, and Popovic}}}
\bibcite{munter}{{21}{1990}{{MUNTER}}{{}}}
\global \chardef \firstnote@num21\relax 
\bibstyle{apsrev}
\newlabel{LastPage}{{}{4}}
\newlabel{LastBibItem}{{21}{5}{}{}{}}

